Flexible coinductive logic programming

Recursive definitions of predicates are usually interpreted either inductively or coinductively. Recently, a more powerful approach has been proposed, called flexible coinduction, to express a variety of intermediate interpretations, necessary in some cases to get the correct meaning. We provide a detailed formal account of an extension of logic programming supporting flexible coinduction. Syntactically, programs are enriched by coclauses, clauses with a special meaning used to tune the interpretation of predicates. As usual, the declarative semantics can be expressed as a fixed point which, however, is not necessarily the least, nor the greatest one, but is determined by the coclauses. Correspondingly, the operational semantics is a combination of standard SLD resolution and coSLD resolution. We prove that the operational semantics is sound and complete with respect to declarative semantics restricted to finite comodels. This paper is under consideration for acceptance in TPLP.

==> ltl-example.tex <==
\subsubsection*{An LTL fragment}
\begin{lstlisting}[basicstyle=\ttfamily\small]
%%% words must be infinite 
infinite([B|W]) $\clSep$ infinite(W)
infinite([B|W]) $\clSep$ infinite(W)
infinite(W) $\coclSep$

%%% formulae must be finite 
finite(zero) $\clSep$
finite(one) $\clSep$
finite(always(Ph)) $\clSep$ finite(Ph)
finite(until(Ph1,Ph2)) $\clSep$ finite(Ph1), finite(Ph2)

satisfies(W,Ph) $\clSep$ infinite(W),finite(Ph),sat(W,Ph)

sat([0|W],zero) $\clSep$
sat([1|W],one) $\clSep$
sat([B|W],always(Ph)) $\clSep$ sat([B|W],Ph), sat(W,always(Ph)) 
sat(W,always(Ph)) $\coclSep$ sat(W,Ph)
sat([B|W],until(Ph1,Ph2)) $\clSep$ sat([B|W],Ph1), sat(W,until(Ph1,Ph2)) 
sat(W,until(Ph1,Ph2)) $\clSep$ sat(W,Ph2) 
\end{lstlisting}

Traditionally in standard LTL words are infinite, but removing the constraint \lstinline{infinite(W)} from the
body of the definition of \lstinline{satisfies} is not a problem, it would simply allow the interpretation to be extended to finite words.
For instance \lstinline{sat([1,1,0],until(one,zero))} is derivable, while \lstinline{sat([1,1,1],always(one))} is not, as expected.

The atom \lstinline{finite(Ph)} in the
body of the definition of \lstinline{satisfies} requires LTL formulae to be inductive, as expected by definition;
\lstinline{sat(W0,Ph)} is derivable with \lstinline{W0=[0|W0]} and \lstinline{Ph=until(Ph,always(zero))}, and
this fact could be considered reasonable, recursive formulae in LTL are meaningless had have no standard interpretation.

The corule for \lstinline{always} allows derivations of atoms such as \lstinline{sat(W0,always(zero))} with 
\lstinline{W0=[0|W0]}, for which the derivation is always infinite; for \lstinline{always} a corule is needed,
because the cofact \lstinline{sat(W,always(Ph))$\coclSep$} would allow derivation of  \lstinline{sat(W1,until(one,always(zero)))}
with \lstinline{W1=[1|W1]}, which is unsound.

For what concerns the  \lstinline{until} operator, no corule needs to be defined:
\begin{itemize}
\item a corule for  \lstinline{until} is \textbf{not} necessary to derive \lstinline{sat([1,1,0|W1],until(one,zero))} with \lstinline{W1=[1|W1]}, because in this case the only possible derivation is finite;
\item a corule for  \lstinline{until} is \textbf{not} necessary to derive \lstinline{sat([1,1|W0],until(one,always(zero)))} with \lstinline{W0=[0|W0]}, because in this case the only possible derivation is infinite, but corule for \lstinline{always} can be used to build finite derivations for all nodes in the infinite derivation; 
\item absence of a corule for  \lstinline{until} allows atoms such as \lstinline{sat(W1,until(one,zero))}, \lstinline{sat(W1,until(always(one),zero))}
and \lstinline{sat(W1,until(always(one),always(zero)))} not to be derivable with \lstinline{W1=[1|W1]}, as expected. 
\end{itemize} 

